An interferometric view of hot star disks

Optical long baseline interferometry was recently established as a technique capable of resolving stars and their circumstellar environments at the milliarcsecond (mas) resolution level. This high-resolution opens an entire new window to the study of astrophysical systems, providing information inaccessible by other techniques. Astrophysical disks are observed in a wide variety of systems, from galaxies up to planetary rings, commonly sharing similar physical processes. Two particular disk like systems are studied in the thesis: (i) B He-rich stars that exhibits magnetic fields in order of kG and that trap their winds in structures called magnetospheres; and (ii) Be stars, fast rotating stars that create circumstellar viscous disks. This study uses the interferometric technique to investigate both the photosphere proper and the circumstellar environment of these stars. The objective is to combine interferometry with other observational techniques (such as spectroscopy and polarimetry) to perform a complete and well-constrained physical description of these systems. This description is accompanied by radiative transfer models performed by the HDUST code. Keywords: stars: individual (Achernar), stars: fundamental parameters, techniques: interferometric, circumstellar matter, stars: emission-line, Be, stars: magnetic field

==> chap/conclusions.tex <==
% geany_encoding=ISO-8859-15 %#
\chapter{Conclusions and Perspectives \label{chap:conc}}
In this work we performed the study of circumstellar structures of two hot stars subtypes: the magnetospheres of He-rich stars and the viscous disks of the Be stars.

Magnetism is a common feature among hot stars. Among them, some display magnetic fields on the order of tens of kG, trapping the circumstellar wind in a structure called magnetosphere. We held the first polarimetric characterization of a hot star magnetosphere to \sori{}. This study led to a revision in the understanding of these structures hitherto spectroscopically described by RRM model. In this work we present the polarimetric detection for two more magnetospheres, HR\,7355 and HR\,5907. Our results show that this stars have similar polarimetric characteristics, increasing significance for the conclusions obtained for this structures, namely a different density distribution than expected. 

As perspectives in this field, we expect to increase the polarimetric data available in order to increase the accuracy in the parameters determinations and to extend these analyzes to other known magnetic stars. Also, we hope to take a step further studying the light curve proposed by the structures defined from polarimetry solving the problem of radiative transfer, and reassess the latest beam-combiners capacity to map these structures in interferometry (as PIONIER). 

Be stars are important targets to investigate physical processes governing stellar evolution (specially at high rotational rates) and astrophysical viscous disks. The rapid rotation of these stars is fundamentally linked to the existence of the circumstellar disk. Due to their brightness, they can be investigated by multiple observational techniques, notably interferometry. 

Interferometry is sensitive to the brightness distribution of a observed target. The relation of physical properties of Be stars and the interferometric data can only be directly determined if they are analyzed by realistic emission models. Both interferometry and spectrointerferometry allowed establishing the viscous decretion disk (VDD) model, solved by radiative transfer, as the most likely scenario to explain the Be star disks.

The solutions provided by radiative transfer can both determine the structure as well the emergent observables of the Be stars. This enables, for instance, the study of second order effects that may be present on these systems. Multi-technique studies, combining integrated quantities (as photometry or spectroscopy) with ones containing spatial information (as polarimetry or interferometry) are an important way of constraining the multiple parameters that characterized the systems in a consistent way. 
% - and that could be related to the unknown process of the Be phenomenon.

There are still important open issues aimed to be investigated. The VDD model go a long way in describing disk structure and evolution, but lacks in explaining the mass ejection mechanisms by the star and the nature of disk viscosity, key process to the phenomenon occurrence. The VDD model capability in describing the Be stars circumstellar could be seen with some caution. Stringent tests of the VDD with angularly resolved information provided by interferometry were performed only on a handful of stars so far: $\chi$\,Oph, $\kappa$\,Dra, $\beta$\,Psc and $\nu$\,Cyg (\citealp{jon08a, tyc08a}; fit of interferometry and line profiles using a time-independent parametric model); $\zeta$\,Tau and $\delta$\,Sco (\citealp{car06a, car09a}; fit of interferometry, polarimetry, spectroscopy and photometry using time-independent self-consistent model). 

For example, an important effect usually ignored in Be disks is the modifications imposed on disk structure by the tidal effects of a companion star (e.g., \citealp{oka02a}). $\beta$\,CMi is a late-type Be star with a known stable disk. The recent detailed modeling of $\beta$\,CMi by \citep{kle15a} has shown for the first time the influence of a secondary star in a Be disk. The cited study contains a comprehensive observational data set that cover a huge spectral interval. The conclusion is that the disk has a dual density behavior due to the companion, with steeper density in the inner part and shallower density in the outer part. 

%~ The universality of VDD needs to confirmed, as well as the detailed conditions at disk extension. 
In this context, observables with diagnostic potential are important to characterize these systems, as the CQE-PS, as well multiple technique analyses to search for and characterize the second order effects at play in the disk. This reinforces the unique role that the \textsc{BeAtlas} project can play. The parameters range covered will enable the detailed investigation of multiple targets, expanding the Be star radiative-transfer based analysis to statically significant number of targets. The comprehensive quantities predicted will allow building detailed picture of the Be phenomenon in physical terms. 




==> tex/abstrakta.tex <==
Resumo


==> tex/ap-REF.tex <==
% geany_encoding=ISO-8859-15 %
\chapter{Modeling Rotating Stars \label{ap:modrots}}




==> tex/exemplo_tabela_longtable.tex <==
\begin{center}
\setcaptionmargin{1cm}
\scriptsize
\begin{longtable}{lcccc}
\caption[Resumo da legenda da tabela (aparece na lista de figuras)]{Exemplo de tabela feita com o longtable.}\\
\hline \hline \\[-2ex]
\multicolumn{1}{c}{Coluna1} &
\multicolumn{1}{c}{Coluna2} &
\multicolumn{1}{c}{Coluna3} &
\multicolumn{1}{c}{Coluna4} &
\multicolumn{1}{c}{Coluna5} 

\\[0.5ex] \hline
\\[-1.8ex]

\endfirsthead

\multicolumn{5}{c}{\footnotesize{{\slshape{{\tablename} \thetable{}}} - Continuação}}\\[0.5ex]

\hline \hline\\[-2ex]

\multicolumn{1}{c}{Coluna1} &
\multicolumn{1}{c}{Coluna2} &
\multicolumn{1}{c}{Coluna3} &
\multicolumn{1}{c}{Coluna4} &
\multicolumn{1}{c}{Coluna5} 

\\[0.5ex] \hline
\\[-1.8ex]

\endhead

\multicolumn{3}{l}{{\footnotesize{Continua na próxima página\ldots}}}\\
\endfoot
\hline

\endlastfoot

1 & 2 & 3 & 4 & 5 \\
6 & 7 & 8 & 9 & 10\\

\label{tabela_com_longtable}
\end{longtable}
\end{center}



==> tex/listofabbrev.tex <==
% geany_encoding=ISO-8859-15 %

%~ \chapter{List of abbreviations, acronyms and definitions}
\begin{itemize}
\normalsize \setlength\itemsep{-.5pt} %0em
    \item[$\alpha$ :]is the Shakura-Sunyaev viscous parameter
    \item[$\lambda$ :] electromagnetic wavelength
    \item[$\rho$ :]is the volumetric mass density
    \item[$\sigma$ :] free electron cross section
    \item[$\Sigma$ :]is the superficial mass density
    \item[$\tau$ :] optical opacity
    \item[IS :]interstellar
    \item[ISM :]interstellar mediu
    \item[$H$ :] disk scale height
    \item[$n$ :] radial exponent of the superficial disk density
    \item[$m$ :] radial exponent of the volumetric disk density
    \item[$\dot{M}$ :]is the star disk mass injection rate
    \item[$P_{\rm int}$ :]intrinsic polarization
    \item[$P_{\rm obs}$ :]observed polarization
    \item[$R_0$ :]is the disk truncation radius
    \item[$R_{\rm *}$ :] stellar radius. For fast rotators stars, is the equatorial radius
    \item[$R_{\rm eq}$ :] stellar equatorial radius
    \item[$R_{\rm p}$ :] stellar polar radius
    \item[$v_{\rm eq}$ :] is the disk orbital speed at the stellar equatorial radius
    \item[$v_s$ :]is the sound speed
    \item[$z$ :]is the vertical coordinate in the cylindrical system
\end{itemize}
{\color{orange} TODO to be completed and organized}

